Fairify: Fairness Verification of Neural Networks

Fairness of machine learning (ML) software has become a major concern in the recent past. Although recent research on testing and improving fairness have demonstrated impact on real-world software, providing fairness guarantee in practice is still lacking. Certification of ML models is challenging because of the complex decision-making process of the models. In this paper, we proposed Fairify, an SMT-based approach to verify individual fairness property in neural network (NN) models. Individual fairness ensures that any two similar individuals get similar treatment irrespective of their protected attributes e.g., race, sex, age. Verifying this fairness property is hard because of the global checking and non-linear computation nodes in NN. We proposed sound approach to make individual fairness verification tractable for the developers. The key idea is that many neurons in the NN always remain inactive when a smaller part of the input domain is considered. So, Fairify leverages whitebox access to the models in production and then apply formal analysis based pruning. Our approach adopts input partitioning and then prunes the NN for each partition to provide fairness certification or counterexample. We leveraged interval arithmetic and activation heuristic of the neurons to perform the pruning as necessary. We evaluated Fairify on 25 real-world neural networks collected from four different sources, and demonstrated the effectiveness, scalability and performance over baseline and closely related work. Fairify is also configurable based on the domain and size of the NN. Our novel formulation of the problem can answer targeted verification queries with relaxations and counterexamples, which have practical implications.

==> baseline.tex <==



% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
    \centering
    \scriptsize
    \setlength\tabcolsep{1.8pt}
    \caption{The baseline for fairness verification of DNN. B: Baseline, B w/ P: Baseline with partitioning.}
      \begin{tabular}{lllllllllllllllllllllllllllllllll}
      \hline
      \textbf{PA} & \multicolumn{8}{c|}{\textbf{Age}}                             & \multicolumn{5}{c|}{\textbf{Sex}}     & \multicolumn{5}{c|}{\textbf{Race}}    & \multicolumn{7}{c|}{\textbf{Race}}                    & \multicolumn{7}{c}{\textbf{Sex}} \\
      \hline
      \textbf{Model} & \textbf{BM1} & \textbf{BM2} & \textbf{BM3} & \textbf{BM4} & \textbf{BM5} & \textbf{BM6} & \textbf{BM7} & \textbf{BM8} & \textbf{GC1} & \textbf{GC2} & \textbf{GC3} & \textbf{GC4} & \textbf{GC5} & \textbf{GC1} & \textbf{GC2} & \textbf{GC3} & \textbf{GC4} & \textbf{GC5} & \textbf{AC1} & \textbf{AC2} & \textbf{AC3} & \textbf{AC4} & \textbf{AC5} & \textbf{AC6} & \textbf{AC7} & \textbf{AC1} & \textbf{AC2} & \textbf{AC3} & \textbf{AC4} & \textbf{AC5} & \textbf{AC6} & \textbf{AC7} \\
      \hline
      \textbf{B} & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & - \\
      \textbf{B w/ P} & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & - \\
      \hline
      \end{tabular}%
    \label{tab:baseline}%
  \end{table*}%



==> discussion.tex <==
\section{Discussion}
\label{sec:disc}

With the increase of data intensive software usage, it has been critical to ensure the fairness of the software in the wild. \citeauthor{brun2018software} argued that we are still in an early stage to understand fairness problems and solve it effectively. We need further tools, method, and approaches to test, verify and reason about fairness in software systems \cite{brun2018software}. In this paper, we are the first, to verify deep neural networks effectively on a wide number of deep neural networks. Our results also show further possibility in research to address the fairness issue in software.

\begin{enumerate}[leftmargin=*]
    \item Software verification and testing methodologies can be considered together. For example, \citeauthor{aggarwal2019black} leveraged symbolic execution for input test case generation \cite{aggarwal2019black}. We envision fairness verification as a technique to generate seed counterexamples that can be used to find more test inputs for the software. 
    
    \item In our approach, we used lightweight technique to find the neurons that are inactive. leveraging domain specific knowledge such as identifying the attributes that affects the decision more than others, can guide selecting more neurons for pruning. 
    
    \item We used to create a number of partitioning before starting the actual verification. Can we use partitioning on-the-fly based on other heuristics, or earlier verification results?
\end{enumerate}


==> libra-table.tex <==

\begin{table}[t]
  \footnotesize
  \setlength\tabcolsep{2.05pt}
  \centering
  % \vspace{3pt}
  \caption{Verification for the models in \cite{urban2020perfectly} on AC dataset. Total \#P: 432, |M|: \#hidden neurons, time {\tiny\VarClock} in seconds.}
    \begin{tabular}{|ccrrrrrrrr|}
    \hline
    \rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{|l}{\textbf{|M|}} & \textbf{Ver} & \multicolumn{1}{l}{\textbf{\#P}} & \multicolumn{1}{l}{\textbf{Coverage}} & \multicolumn{1}{l}{\textbf{\#sat}} & \multicolumn{1}{l}{\textbf{\#unsat}} & \multicolumn{1}{l}{\textbf{\#unk}} & \multicolumn{1}{l}{\textbf{SV {\tiny\VarClock}}} & \multicolumn{1}{l}{\textbf{HV {\tiny\VarClock}}} & \multicolumn{1}{l|}{\textbf{Total {\tiny\VarClock}}} \\
    % \hline
    10    & SAT   & 178      & 41.20\% & 157      & 21      & 0      & 19.84      & 0.29      & 20.24 \\
    \rowcolor[rgb]{ .949,  .949,  .949} 12    & SAT   & 432   & 100.00\% & 231   & 201   & 0     & 4.12  & 0.00  & 4.23 \\
    20    & SAT   & 39    & 7.64\% & 11    & 22    & 6     & 64.20 & 31.77 & 96.12 \\
    \rowcolor[rgb]{ .949,  .949,  .949} 40    & UNK   & 9     & 0.00\% & 0     & 0     & 9     & 200.32 & 200.26 & 401.02 \\
    45    & SAT   & 29    & 4.63\% & 1     & 19    & 9     & 69.95 & 66.95 & 137.12 \\
    \hline
  \end{tabular}%
\label{tab:libra}%
% \vspace{-5.6mm}
\end{table}%



==> old-table.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
    \centering
    \footnotesize
    \setlength\tabcolsep{2.8pt}
    \caption{Fairness verification results. For all the models, we used 100s soft-timeout. The hard-timeout was 30m for BM and GC models, and 60m for AC models. 
  V: Verification, \#P: number of partition, \#H-At: number of time heuristic pruning attempted, CP: average compression ratio, S: sound pruning, H: heuristic pruning, S-time: solving time (average), T-time: total time (average)}
      \begin{tabular}{|c|l|r|r|l|r|r|r|r|r|r|r|r|r|r|}
      \hline
      \rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{|l|}{\textbf{PA}} & \textbf{Model} & \multicolumn{1}{l|}{\textbf{Base-V}} & \multicolumn{1}{l|}{\textbf{Base-P}} & \textbf{V} & \multicolumn{1}{l|}{\textbf{\#P}} & \multicolumn{1}{l|}{\textbf{\#SAT}} & \multicolumn{1}{l|}{\textbf{\#UNSAT}} & \multicolumn{1}{l|}{\textbf{\#UNK}} & \multicolumn{1}{l|}{\textbf{\#H-At}} & \multicolumn{1}{l|}{\textbf{CP-S}} & \multicolumn{1}{l|}{\textbf{CP-H}} & \multicolumn{1}{l|}{\textbf{S-time}} & \multicolumn{1}{l|}{\textbf{T-time}} & \multicolumn{1}{l|}{\textbf{Acc $\downarrow$ }} \\
      \hline
      \multirow{8}[2]{*}{\begin{sideways}Age\end{sideways}} & BM1   & UNK   & UNK   & SAT   & 127   & 18    & 94    & 15    & 16    & 89.88 & 0.67  & 7.10  & 14.01 & 1.16 \\
            & \cellcolor[rgb]{ .949,  .949,  .949}BM2 & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}SAT & \cellcolor[rgb]{ .949,  .949,  .949}171 & \cellcolor[rgb]{ .949,  .949,  .949}121 & \cellcolor[rgb]{ .949,  .949,  .949}11 & \cellcolor[rgb]{ .949,  .949,  .949}0 & \cellcolor[rgb]{ .949,  .949,  .949}16 & \cellcolor[rgb]{ .949,  .949,  .949}85.55 & \cellcolor[rgb]{ .949,  .949,  .949}1.05 & \cellcolor[rgb]{ .949,  .949,  .949}4.88 & \cellcolor[rgb]{ .949,  .949,  .949}10.03 & \cellcolor[rgb]{ .949,  .949,  .949}1.17 \\
            & BM3   & UNK   & UNK   & SAT   & 174   & 36    & 124   & 14    & 16    & 96.52 & 0.19  & 5.12  & 10.28 & 0.00 \\
            & \cellcolor[rgb]{ .949,  .949,  .949}BM4 & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}SAT & \cellcolor[rgb]{ .949,  .949,  .949}19 & \cellcolor[rgb]{ .949,  .949,  .949}2 & \cellcolor[rgb]{ .949,  .949,  .949}12 & \cellcolor[rgb]{ .949,  .949,  .949}5 & \cellcolor[rgb]{ .949,  .949,  .949}5 & \cellcolor[rgb]{ .949,  .949,  .949}83.79 & \cellcolor[rgb]{ .949,  .949,  .949}5.18 & \cellcolor[rgb]{ .949,  .949,  .949}13.98 & \cellcolor[rgb]{ .949,  .949,  .949}93.10 & \cellcolor[rgb]{ .949,  .949,  .949}0.02 \\
            & BM5   & UNK   & UNK   & SAT   & 510   & 108   & 394   & 8     & 0     & 82.54 & 0.19  & 1.61  & 2.94  & 0.49 \\
            & \cellcolor[rgb]{ .949,  .949,  .949}BM6 & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}SAT & \cellcolor[rgb]{ .949,  .949,  .949}510 & \cellcolor[rgb]{ .949,  .949,  .949}154 & \cellcolor[rgb]{ .949,  .949,  .949}354 & \cellcolor[rgb]{ .949,  .949,  .949}2 & \cellcolor[rgb]{ .949,  .949,  .949}4 & \cellcolor[rgb]{ .949,  .949,  .949}76.01 & \cellcolor[rgb]{ .949,  .949,  .949}0.20 & \cellcolor[rgb]{ .949,  .949,  .949}1.10 & \cellcolor[rgb]{ .949,  .949,  .949}1.72 & \cellcolor[rgb]{ .949,  .949,  .949}4.43 \\
            & BM7   & UNK   & UNK   & SAT   & 152   & 64    & 81    & 7     & 12    & 91.33 & 0.94  & 4.79  & 11.84 & 1.35 \\
            & \cellcolor[rgb]{ .949,  .949,  .949}BM8 & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}SAT & \cellcolor[rgb]{ .949,  .949,  .949}27 & \cellcolor[rgb]{ .949,  .949,  .949}3 & \cellcolor[rgb]{ .949,  .949,  .949}21 & \cellcolor[rgb]{ .949,  .949,  .949}3 & \cellcolor[rgb]{ .949,  .949,  .949}4 & \cellcolor[rgb]{ .949,  .949,  .949}0.84 & \cellcolor[rgb]{ .949,  .949,  .949}0.01 & \cellcolor[rgb]{ .949,  .949,  .949}47.30 & \cellcolor[rgb]{ .949,  .949,  .949}86.39 & \cellcolor[rgb]{ .949,  .949,  .949}0.36 \\
      \hline \hline
      \multirow{5}[2]{*}{\begin{sideways}Sex\end{sideways}} & GC1   & UNK   & UNK   & SAT   & 34    & 25    & 0     & 9     & 17    & 75.49 & 2.13  & 26.43 & 52.54 & 0.00 \\
            & \cellcolor[rgb]{ .949,  .949,  .949}GC2 & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}SAT & \cellcolor[rgb]{ .949,  .949,  .949}18 & \cellcolor[rgb]{ .949,  .949,  .949}1 & \cellcolor[rgb]{ .949,  .949,  .949}0 & \cellcolor[rgb]{ .949,  .949,  .949}17 & \cellcolor[rgb]{ .949,  .949,  .949}17 & \cellcolor[rgb]{ .949,  .949,  .949}79.87 & \cellcolor[rgb]{ .949,  .949,  .949}3.85 & \cellcolor[rgb]{ .949,  .949,  .949}49.79 & \cellcolor[rgb]{ .949,  .949,  .949}99.14 & \cellcolor[rgb]{ .949,  .949,  .949}0.00 \\
            & GC3   & UNK   & UNK   & SAT   & 201   & 193   & 6     & 2     & 2     & 69.40 & 0.10  & 1.68  & 2.87  & 0.00 \\
            & \cellcolor[rgb]{ .949,  .949,  .949}GC4 & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}SAT & \cellcolor[rgb]{ .949,  .949,  .949}201 & \cellcolor[rgb]{ .949,  .949,  .949}2 & \cellcolor[rgb]{ .949,  .949,  .949}198 & \cellcolor[rgb]{ .949,  .949,  .949}1 & \cellcolor[rgb]{ .949,  .949,  .949}1 & \cellcolor[rgb]{ .949,  .949,  .949}63.32 & \cellcolor[rgb]{ .949,  .949,  .949}0.09 & \cellcolor[rgb]{ .949,  .949,  .949}0.59 & \cellcolor[rgb]{ .949,  .949,  .949}1.68 & \cellcolor[rgb]{ .949,  .949,  .949}0.00 \\
            & GC5   & UNK   & UNK   & UNK   & 21    & 0     & 4     & 17    & 17    & 61.60 & 3.47  & 40.78 & 83.22 & 0.00 \\
      \hline
      \multirow{5}[2]{*}{\begin{sideways}Age\end{sideways}} & \cellcolor[rgb]{ .949,  .949,  .949}GC1 & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}SAT & \cellcolor[rgb]{ .949,  .949,  .949}39 & \cellcolor[rgb]{ .949,  .949,  .949}31 & \cellcolor[rgb]{ .949,  .949,  .949}0 & \cellcolor[rgb]{ .949,  .949,  .949}8 & \cellcolor[rgb]{ .949,  .949,  .949}17 & \cellcolor[rgb]{ .949,  .949,  .949}75.82 & \cellcolor[rgb]{ .949,  .949,  .949}1.71 & \cellcolor[rgb]{ .949,  .949,  .949}25.73 & \cellcolor[rgb]{ .949,  .949,  .949}44.88 & \cellcolor[rgb]{ .949,  .949,  .949}0.00 \\
            & GC2   & UNK   & UNK   & SAT   & 19    & 5     & 0     & 14    & 16    & 80.20 & 3.60  & 46.53 & 90.86 & 0.00 \\
            & \cellcolor[rgb]{ .949,  .949,  .949}GC3 & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}SAT & \cellcolor[rgb]{ .949,  .949,  .949}201 & \cellcolor[rgb]{ .949,  .949,  .949}199 & \cellcolor[rgb]{ .949,  .949,  .949}0 & \cellcolor[rgb]{ .949,  .949,  .949}2 & \cellcolor[rgb]{ .949,  .949,  .949}2 & \cellcolor[rgb]{ .949,  .949,  .949}69.40 & \cellcolor[rgb]{ .949,  .949,  .949}0.10 & \cellcolor[rgb]{ .949,  .949,  .949}1.67 & \cellcolor[rgb]{ .949,  .949,  .949}2.94 & \cellcolor[rgb]{ .949,  .949,  .949}0.00 \\
            & GC4   & UNK   & UNK   & SAT   & 201   & 200   & 1     & 0     & 1     & 63.32 & 0.09  & 0.42  & 1.59  & 0.00 \\
            & \cellcolor[rgb]{ .949,  .949,  .949}GC5 & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}23 & \cellcolor[rgb]{ .949,  .949,  .949}0 & \cellcolor[rgb]{ .949,  .949,  .949}6 & \cellcolor[rgb]{ .949,  .949,  .949}17 & \cellcolor[rgb]{ .949,  .949,  .949}17 & \cellcolor[rgb]{ .949,  .949,  .949}59.23 & \cellcolor[rgb]{ .949,  .949,  .949}3.69 & \cellcolor[rgb]{ .949,  .949,  .949}37.42 & \cellcolor[rgb]{ .949,  .949,  .949}76.77 & \cellcolor[rgb]{ .949,  .949,  .949}0.00 \\
      \hline \hline
      \multirow{7}[2]{*}{\begin{sideways}Race\end{sideways}} & AC1   & UNK   & UNK   & SAT   & 39    & 7     & 19    & 13    & 17    & 64.82 & 4.51  & 44.32 & 89.08 & -2.26 \\
            & \cellcolor[rgb]{ .949,  .949,  .949}AC2 & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}SAT & \cellcolor[rgb]{ .949,  .949,  .949}43 & \cellcolor[rgb]{ .949,  .949,  .949}18 & \cellcolor[rgb]{ .949,  .949,  .949}13 & \cellcolor[rgb]{ .949,  .949,  .949}12 & \cellcolor[rgb]{ .949,  .949,  .949}14 & \cellcolor[rgb]{ .949,  .949,  .949}88.47 & \cellcolor[rgb]{ .949,  .949,  .949}0.99 & \cellcolor[rgb]{ .949,  .949,  .949}48.39 & \cellcolor[rgb]{ .949,  .949,  .949}83.02 & \cellcolor[rgb]{ .949,  .949,  .949}1.09 \\
            & AC3   & UNK   & UNK   & SAT   & 44    & 32    & 0     & 12    & 15    & 77.98 & 1.29  & 42.93 & 78.39 & 4.11 \\
            & \cellcolor[rgb]{ .949,  .949,  .949}AC4 & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}SAT & \cellcolor[rgb]{ .949,  .949,  .949}15 & \cellcolor[rgb]{ .949,  .949,  .949}2 & \cellcolor[rgb]{ .949,  .949,  .949}0 & \cellcolor[rgb]{ .949,  .949,  .949}13 & \cellcolor[rgb]{ .949,  .949,  .949}14 & \cellcolor[rgb]{ .949,  .949,  .949}79.54 & \cellcolor[rgb]{ .949,  .949,  .949}9.29 & \cellcolor[rgb]{ .949,  .949,  .949}94.16 & \cellcolor[rgb]{ .949,  .949,  .949}232.56 & \cellcolor[rgb]{ .949,  .949,  .949}0.25 \\
            & AC5   & UNK   & UNK   & SAT   & 17    & 2     & 0     & 15    & 17    & 76.72 & 2.20  & 92.17 & 205.53 & 1.58 \\
            & \cellcolor[rgb]{ .949,  .949,  .949}AC6 & \cellcolor[rgb]{ .949,  .949,  .949}SAT & \cellcolor[rgb]{ .949,  .949,  .949}SAT & \cellcolor[rgb]{ .949,  .949,  .949}SAT & \cellcolor[rgb]{ .949,  .949,  .949}40 & \cellcolor[rgb]{ .949,  .949,  .949}15 & \cellcolor[rgb]{ .949,  .949,  .949}9 & \cellcolor[rgb]{ .949,  .949,  .949}16 & \cellcolor[rgb]{ .949,  .949,  .949}16 & \cellcolor[rgb]{ .949,  .949,  .949}56.90 & \cellcolor[rgb]{ .949,  .949,  .949}3.70 & \cellcolor[rgb]{ .949,  .949,  .949}48.31 & \cellcolor[rgb]{ .949,  .949,  .949}89.56 & \cellcolor[rgb]{ .949,  .949,  .949}2.00 \\
            & AC7   & UNK   & UNK   & UNK   & 23    & 0     & 10    & 13    & 17    & 60.63 & 9.36  & 70.69 & 152.25 & 2.34 \\
      \hline 
      \multirow{7}[2]{*}{\begin{sideways}Sex\end{sideways}} & \cellcolor[rgb]{ .949,  .949,  .949}AC1 & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}SAT & \cellcolor[rgb]{ .949,  .949,  .949}47 & \cellcolor[rgb]{ .949,  .949,  .949}3 & \cellcolor[rgb]{ .949,  .949,  .949}28 & \cellcolor[rgb]{ .949,  .949,  .949}16 & \cellcolor[rgb]{ .949,  .949,  .949}17 & \cellcolor[rgb]{ .949,  .949,  .949}66.47 & \cellcolor[rgb]{ .949,  .949,  .949}4.94 & \cellcolor[rgb]{ .949,  .949,  .949}38.56 & \cellcolor[rgb]{ .949,  .949,  .949}75.90 & \cellcolor[rgb]{ .949,  .949,  .949}0.03 \\
            & AC2   & UNK   & UNK   & SAT   & 30    & 10    & 6     & 14    & 15    & 85.58 & 1.82  & 65.06 & 117.39 & 1.14 \\
            & \cellcolor[rgb]{ .949,  .949,  .949}AC3 & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}SAT & \cellcolor[rgb]{ .949,  .949,  .949}48 & \cellcolor[rgb]{ .949,  .949,  .949}39 & \cellcolor[rgb]{ .949,  .949,  .949}0 & \cellcolor[rgb]{ .949,  .949,  .949}9 & \cellcolor[rgb]{ .949,  .949,  .949}14 & \cellcolor[rgb]{ .949,  .949,  .949}77.69 & \cellcolor[rgb]{ .949,  .949,  .949}1.76 & \cellcolor[rgb]{ .949,  .949,  .949}44.13 & \cellcolor[rgb]{ .949,  .949,  .949}74.73 & \cellcolor[rgb]{ .949,  .949,  .949}3.63 \\
            & AC4   & UNK   & UNK   & SAT   & 13    & 2     & 0     & 11    & 12    & 68.85 & 17.68 & 98.48 & 273.31 & -0.09 \\
            & \cellcolor[rgb]{ .949,  .949,  .949}AC5 & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}SAT & \cellcolor[rgb]{ .949,  .949,  .949}16 & \cellcolor[rgb]{ .949,  .949,  .949}1 & \cellcolor[rgb]{ .949,  .949,  .949}0 & \cellcolor[rgb]{ .949,  .949,  .949}15 & \cellcolor[rgb]{ .949,  .949,  .949}16 & \cellcolor[rgb]{ .949,  .949,  .949}71.90 & \cellcolor[rgb]{ .949,  .949,  .949}10.95 & \cellcolor[rgb]{ .949,  .949,  .949}0.83 & \cellcolor[rgb]{ .949,  .949,  .949}97.43 & \cellcolor[rgb]{ .949,  .949,  .949}0.98 \\
            & AC6   & UNK   & UNK   & SAT   & 33    & 12    & 7     & 14    & 33    & 54.91 & 4.61  & 51.74 & 104.54 & 1.95 \\
            & \cellcolor[rgb]{ .949,  .949,  .949}AC7 & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}UNK & \cellcolor[rgb]{ .949,  .949,  .949}21 & \cellcolor[rgb]{ .949,  .949,  .949}0 & \cellcolor[rgb]{ .949,  .949,  .949}8 & \cellcolor[rgb]{ .949,  .949,  .949}13 & \cellcolor[rgb]{ .949,  .949,  .949}20 & \cellcolor[rgb]{ .949,  .949,  .949}57.49 & \cellcolor[rgb]{ .949,  .949,  .949}10.32 & \cellcolor[rgb]{ .949,  .949,  .949}80.01 & \cellcolor[rgb]{ .949,  .949,  .949}165.20 & \cellcolor[rgb]{ .949,  .949,  .949}5.99 \\
      \hline
      \end{tabular}%
    \label{tab:utility}%
  \end{table*}%
